Aya Vision: Advancing the Frontier of Multilingual Multimodality

Building multimodal language models is fundamentally challenging: it requires aligning vision and language modalities, curating high-quality instruction data, and avoiding the degradation of existing text-only capabilities once vision is introduced. These difficulties are further magnified in the multilingual setting, where the need for multimodal data in different languages exacerbates existing data scarcity, machine translation often distorts meaning, and catastrophic forgetting is more pronounced. To address the aforementioned challenges, we introduce novel techniques spanning both data and modeling. First, we develop a synthetic annotation framework that curates high-quality, diverse multilingual multimodal instruction data, enabling Aya Vision models to produce natural, human-preferred responses to multimodal inputs across many languages. Complementing this, we propose a cross-modal model merging technique that mitigates catastrophic forgetting, effectively preserving text-only capabilities while simultaneously enhancing multimodal generative performance. Aya-Vision-8B achieves best-in-class performance compared to strong multimodal models such as Qwen-2.5-VL-7B, Pixtral-12B, and even much larger Llama-3.2-90B-Vision. We further scale this approach with Aya-Vision-32B, which outperforms models more than twice its size, such as Molmo-72B and LLaMA-3.2-90B-Vision. Our work advances multilingual progress on the multi-modal frontier, and provides insights into techniques that effectively bend the need for compute while delivering extremely high performance.

==> tables/translation_examples.tex <==
\definecolor{highlightcolor}{RGB}{240, 243, 250}
\definecolor{framecolor}{RGB}{83, 109, 222}




\begin{tcolorbox}[
    colback=highlightcolor!90, 
    colframe=framecolor, 
    boxrule=0.8pt, 
    title=Hindi,
]

  % \noindent
  \adjustbox{valign=t}{
  \begin{minipage}[t]{0.45\textwidth}
    \includegraphics[width=0.6\linewidth]{images/translation_example_1_vqav2.png} \\
    \footnotesize{VQAv2 \citep{goyal2017making}}
  \end{minipage}
  }
  % \hfill
  % \noindent
  \adjustbox{valign=t}{
  \begin{minipage}[t]{0.5\textwidth}
    \textcolor{blue}{\textbf{Prompt}} \\
    Has the kitchen been recently renovated? \\
    \textcolor{blue}{\textbf{NLLB Translated Prompt}} \\
    \begin{hindi}क्या रसोईघर का हाल ही में नवीनीकरण किया गया है? \end{hindi} \\
    \textcolor{blue}{\textbf{Rephrased Prompt}} \\
    \begin{hindi}क्या हाल ही में रसोई का नवीनीकरण किया गया है? \end{hindi} 
  \end{minipage}
  } \\
  
    % \vspace{1pt}
    \hrulefill

    \textcolor{blue}{\textbf{Recaption}} \\
    No, the kitchen has not been recently renovated. The presence of an older model refrigerator, the worn countertop with visible stains, and the outdated wallpaper suggest that the kitchen is quite aged and has not undergone recent updates or renovations.

    \textcolor{blue}{\textbf{NLLB Translated Recaption}} \\
    \begin{hindi}नहीं, रसोई का हाल ही में नवीनीकरण नहीं किया गया है। पुराने मॉडल के रेफ्रिजरेटर की उपस्थिति, दिखने वाले दागों के साथ पहना हुआ काउंटरटॉप, और पुराने वॉलपेपर से पता चलता है कि रसोई काफी पुरानी है और हाल ही में अपडेट या नवीनीकरण नहीं किया गया है \end{hindi} 

    \textcolor{blue}{\textbf{Rephrased Recaption}} \\
    \begin{hindi}नहीं, रसोई का हाल ही में नवीनीकरण नहीं किया गया है। उपकरण पुराने हैं, और समग्र सजावट और सतहों पहनने और उम्र के संकेत दिखाते हैं, यह दर्शाता है कि यह एक समय में किसी भी महत्वपूर्ण अद्यतन या सुधार नहीं किया गया है। \end{hindi} 
\end{tcolorbox}



\begin{tcolorbox}[
    colback=highlightcolor!90, 
    colframe=framecolor, 
    boxrule=0.8pt, 
    title=Turkish,
]

  % \noindent
  \adjustbox{valign=t}{
  \begin{minipage}[t]{0.45\textwidth}
    \includegraphics[width=0.6\linewidth]{images/translation_example_4_gqa.png} \\
    \footnotesize{GQA \citep{hudson2019gqa}}
  \end{minipage}
  }
  % \hfill
  % \noindent
  \adjustbox{valign=t}{
  \begin{minipage}[t]{0.5\textwidth}
    \textcolor{blue}{\textbf{Prompt}} \\
    What kind of furniture is behind the chair? \\
    \textcolor{blue}{\textbf{NLLB Translated Prompt}} \\
    \begin{turkish}Sandalyenin arkasında ne tür bir mobilya var?\end{turkish} \\
    \textcolor{blue}{\textbf{Rephrased Prompt}} \\
    \begin{turkish}Sandalyenin arkasında hangi mobilyalar bulunuyor?\end{turkish} 
  \end{minipage}
  } \\
  
    % \vspace{1pt}
    \hrulefill

    \textcolor{blue}{\textbf{Recaption}} \\
    Behind the chair, there is a wooden bookshelf. This bookshelf appears to be filled with various books and possibly other items, indicating it might be a central piece for storage and organization in this room. The shelf is positioned against the wall, adding to the cozy and functional layout of the space.

    \textcolor{blue}{\textbf{NLLB Translated Recaption}} \\
    \begin{turkish}Sandalyenin arkasında, ahşap bir kitaplık var. Bu kitaplık çeşitli kitaplarla ve muhtemelen diğer eşyalarla dolu görünüyor, bu odada depolama ve düzenleme için merkezi bir parça olabileceğini gösteriyor. Raf duvara dayanarak yerleştirilmiştir, mekanın rahat ve işlevsel düzenine katkıda bulunur.\end{turkish} 

    \textcolor{blue}{\textbf{Rephrased Recaption}} \\
    \begin{turkish}Sandalyenin arkasında, ahşap bir kitaplık bulunuyor. Kitaplık, farklı kitaplar ve muhtemelen diğer eşyalarla dolu görünüyor, bu da odadaki depolama ve düzenleme için önemli bir parça olabileceğini gösteriyor. Kitaplık, duvara yaslanmış şekilde konumlandırılmış ve odanın rahat ve kullanışlı düzenine katkıda bulunuyor. \end{turkish} 
\end{tcolorbox}



\begin{tcolorbox}[
    colback=highlightcolor!90, 
    colframe=framecolor, 
    boxrule=0.8pt, 
    title=Turkish,
]

  % \noindent
  \adjustbox{valign=t}{
  \begin{minipage}[t]{0.45\textwidth}
    \includegraphics[width=0.6\linewidth]{images/translation_example_3_cocoqa.png} \\
    \footnotesize{COCOQA \citep{CocoQA} }
  \end{minipage}
  }
  % \hfill
  % \noindent
  \adjustbox{valign=t}{
  \begin{minipage}[t]{0.5\textwidth}
    \textcolor{blue}{\textbf{Prompt}} \\
    What stands in an open field looking upwards? \\
    \textcolor{blue}{\textbf{NLLB Translated Prompt}} \\
    \begin{chinese}在野外,有一只长<unk>鹿高高的站着,抬头看. 长<unk>鹿的长<unk>子和独特的毛皮图案 \end{chinese} \\
    \textcolor{blue}{\textbf{Rephrased Prompt}} \\
    \begin{chinese}什么东西在空旷的田野中仰望天空?\end{chinese} 
  \end{minipage}
  } \\
  
    % \vspace{1pt}
    \hrulefill

    \textcolor{blue}{\textbf{Recaption}} \\
    In the open field, there is a giraffe standing tall and looking upwards. The giraffe's long neck and distinctive coat pattern of dark patches separated by lighter lines are clearly visible. 

    \textcolor{blue}{\textbf{NLLB Translated Recaption}} \\
    \begin{chinese}在野外,有一只长<unk>鹿高高的站着,抬头看. 长<unk>鹿的长<unk>子和独特的毛皮图案 \end{chinese} 

    \textcolor{blue}{\textbf{Rephrased Recaption}} \\
    \begin{chinese}在空旷的田野中, 有一只长颈鹿昂首挺立, 望向天空. 长颈鹿的长脖子和独特的毛皮图案清晰可见, 由深色斑块和浅色线条间隔组成 \end{chinese} 
\end{tcolorbox}
